HATS-7b: A Hot Super Neptune Transiting a Quiet K Dwarf Star

IW ../submit_V2/abstract.txt ( Row 1 Col 1 6:48 Ctrl-K H for help We report the discovery by the HATSouth network of HATS-7b, a transiting Super-Neptune with a mass of 0.120+/-0.012MJ, a radius of 0.563+/-(0.046,0.034)RJ, and an orbital period of 3.1853days. The host star is a moderately bright (V=13.340+/-0.010mag, K_S=10.976+/-0.026mag) K dwarf star with a mass of 0.849+/-0.027Msun , a radius of 0.815+/-(0.049,-0.035)Rsun, and a metallicity of [Fe/H]=+0.250+/-0.080. The star is photometrically quiet to within the precision of the HATSouth measurements and has low RV jitter. HATS-7b is the second smallest radius planet discovered by a wide-field ground-based transit survey, and one of only a handful of Neptune-size planets with mass and radius determined to 10% precision. Theoretical modeling of HATS-7b yields a hydrogen-helium fraction of 18+/-4% (rock-iron core and H2-He envelope), or 9+/-4% (ice core and H2-He envelope), i.e.it has a composition broadly similar to that of Uranus and Neptune, and very different from that of Saturn, which has 75% of its mass in H2-He. Based on a sample of transiting exoplanets with accurately (<20%) determined parameters, we establish approximate power-law relations for the envelopes of the mass-density distribution of exoplanets. HATS-7b, which, together with the recently discovered HATS-8b, is one of the first two transiting super-Neptunes discovered in the Southern sky, is a prime target for additional follow-up observations with Southern hemisphere facilities to characterize the atmospheres of Super-Neptunes (which we define as objects with mass greater than that of Neptune, and smaller than halfway between that of Neptune and Saturn, i.e. 0.054 MJ<Mp<0.18 MJ).

==> Makefile <==
TARGET		=	hats7
PRINTER		=	waldorf
SUB			=	submit_v1
CURRENTDIR	=	$(shell pwd | sed -e 's|.*/||g')
VERSION		=	$(shell ls -l $(TARGET).tex | \
				sed -e 's|.*->||g' -e 's|.*_V||g' -e 's|.tex||g')
IMAGES		=	$(shell ls img/*.eps)

.PHONY: all clean save print show

all: $(TARGET).pdf

show:
	@echo VERSION: $(VERSION)

$(TARGET).dvi: *.tex *.cls *.bib $(IMAGES)
	sed -e "s|HATVERSION|$(VERSION)|g" emulateapj_template.cls > emulateapj.cls
	latex $(TARGET).tex
	latex $(TARGET).tex
	bibtex $(TARGET)
	latex $(TARGET).tex
	latex $(TARGET).tex
	latex $(TARGET).tex

$(TARGET).ps: $(TARGET).dvi
	dvips -t letter $(TARGET).dvi -o

$(TARGET).pdf: $(TARGET).ps
	ps2pdf $< $@

save:
	tar cvzf ../$(TARGET)_V$(VERSION).tgz ../$(CURRENTDIR)/
	#gzip $(TARGET).tar
	#mv $(TARGET).tar.gz $(TARGET).tgz

sub:
	test -d $(SUB) || mkdir $(SUB)
	test -d $(SUB)/img || mkdir $(SUB)/img
	cp $(TARGET).tex $(SUB)/hatpxx.tex
	cp img/*.eps $(SUB)/img

clean:
	rm -f $(TARGET).ps \
		$(TARGET).dvi \
		$(TARGET).aux \
		$(TARGET).log \
		$(TARGET).pdf \
		$(TARGET).idx \
		$(TARGET).inx \
		$(TARGET).toc \
		$(TARGET).tgz
	
print: $(TARGET).ps
	lpr -P$(PRINTER) $<
	

